Succinct Classical Verification of Quantum Computation

We construct a classically verifiable succinct interactive argument for quantum computation (BQP) with communication complexity and verifier runtime that are poly-logarithmic in the runtime of the BQP computation (and polynomial in the security parameter). Our protocol is secure assuming the post-quantum security of indistinguishability obfuscation (iO) and Learning with Errors (LWE). This is the first succinct argument for quantum computation in the plain model; prior work (Chia-Chung-Yamakawa, TCC '20) requires both a long common reference string and non-black-box use of a hash function modeled as a random oracle. At a technical level, we revisit the framework for constructing classically verifiable quantum computation (Mahadev, FOCS '18). We give a self-contained, modular proof of security for Mahadev's protocol, which we believe is of independent interest. Our proof readily generalizes to a setting in which the verifier's first message (which consists of many public keys) is compressed. Next, we formalize this notion of compressed public keys; we view the object as a generalization of constrained/programmable PRFs and instantiate it based on indistinguishability obfuscation. Finally, we compile the above protocol into a fully succinct argument using a (sufficiently composable) succinct argument of knowledge for NP. Using our framework, we achieve several additional results, including - Succinct arguments for QMA (given multiple copies of the witness), - Succinct non-interactive arguments for BQP (or QMA) in the quantum random oracle model, and - Succinct batch arguments for BQP (or QMA) assuming post-quantum LWE (without iO).

==> 6-succinct-measurement.tex <==
\section{A Verifier-Succinct Measurement Protocol}

In this section, we construct a verifier-succinct $N$-qubit commit-and-measure protocol (\cref{sec:measurement-protocol-definition}) assuming iO and LWE. By verifier-succinct, we mean that all verifier messages can be computed in time $\poly(\secp, \log N)$, while the verifier can compute its final output (i.e., the $\Test(\cdot)$ and $\Out(\cdot)$ algorithms) in time $\poly(\secp, N)$, and the prover messages can have length $\poly(\secp, N)$. We will achieve this succinctness notion for any verifier basis choice $h$ that is the truth table of a small circuit $C: [N]\to \{0,1\}$. 

Our protocol is a variant of the Mahadev protocol~\cite{FOCS:Mahadev18a} in which the verifier's first message $(\pk_1, \hdots, \pk_N)$ is replaced by the output $\PK$ of some batch key generation procedure.\footnote{By this, we mean a tuple $(\Setup, \extpk, \extsk, \Program)$ satisfying all definitions of \cref{def:succinct-key-gen} except for succinctness.} As described in \cref{sec:succinct-clawfree}, we make use of the following properties of the Mahadev rTCFs obtained from batch key generation:

\begin{itemize}
    \item Pseudoindependence (\cref{lemma:pseudoindependence})
    \item Key indistinguishability (Property (3) of \cref{def:succinct-key-gen})
    \item Collapsing of $f_{\pk_j}$ given $\PK$ and all other secret keys $(\sk_i)_{i\neq j}$ (\cref{lemma:io-collapsing}).
    \item Adaptive hardcore bit property of $f_{\pk_j}$ given $\PK$ and all other secret keys $(\sk_i)_{i\neq j}$ (\cref{lemma:io-hardcore-bit}). 
    \item Computational injectivity of $f_{\pk_j}$ when $\pk_j$ is sampled in injective mode, even given $\PK$ and all secret keys (\cref{lemma:io-injectivity}).
    \item Computational two-to-oneness of $f_{\pk_j}$ when $\pk_j$ is sampled in two-to-one mode, even given $\PK$ and all secret keys (\cref{lemma:io-two-to-one}). \alex{Add to previous section}
\end{itemize}

If the batch key generation procedure is \emph{succinct} (\cref{def:succinct-key-gen}), the resulting protocol is verifier-succinct. Using the trivial ``$N$ independent keys'' batch key generation procedure, we recover an analysis of the original \cite{FOCS:Mahadev18a} protocol. 

\subsection{Mahadev's Protocol}\label{subsec:meas-protocol}
Let $\mathsf{ClawFree} = (\Gen, \Eval, \Invert, \Check, \Good)$ denote a family of \cite{FOCS:Mahadev18a} randomized TCFs (\cref{def:clawfree}). For simplicity of the analysis, we assume that on a fixed security parameter~$1^\secp$, $\Gen$ outputs keys defining functions from $\{0,1\} \times D$ to $R$, where $D$ is a fixed-size subset of $\{0,1\}^{\ell(\secp)}$ independent of $\pk$.\footnote{The LWE-based instantiation from \cite{FOCS:BCMVV18} satisfies this property. However, with more complicated expressions, our proof should go through without this simplifying assumption.} We denote the size of $D$ by $L(\secp)$. Let $\mathsf{BatchGen} = (\Setup, \extpk, \extsk, \Program)$ denote a (succinct) batch key generation algorithm for $\Gen$ (\cref{def:succinct-key-gen}). 

We now describe a (verifier-succinct) commit-and-measure protocol $\MP$ using these two building blocks by adapting the \cite{FOCS:Mahadev18a} construction.  

For simplicity, we assume the honest prover $P$ has an $N$-qubit pure state of the form
\[\ket{\psi}_{\RegW} = \sum_{w_1, \hdots, w_N}\alpha_{w_1, \hdots, w_N} \ket{w_1 \hdots w_N}
\]
on its internal $N$-qubit register $\RegW$; the protocol completeness immediately extends to mixed states by linearity. The verifier has a basis string $h\in\{0,1\}^N$, represented by a circuit $C: [N] \rightarrow \{0,1\}$, and wants to obtain a measurement of $\ket{\psi}$ in this basis (where $h_i = 0$ denotes a standard basis measurement and $h_i = 1$ denotes a Hadamard basis measurement). The protocol $\MP$ (for measurement protocol), with prover algorithm $P = (\MP.\Commit, \MP.\Open)$ and verifier algorithm $V = (\MP.\Gen, \MP.\Test, \MP.\Out)$, is executed as follows. 

  

\begin{itemize}
    \item $\MP.\Gen$: On input $1^\secp$ and $N$, the verifier samples a representation of $N$ TCF key pairs by computing $(\PK, \SK) \gets \Setup(1^\secp, N, C)$, where $C$ is circuit computing $C(i) = h_i$. The verifier sends $\PK$ to the prover.
    \item $\MP.\Commit$: Given $\PK$ and its input state $\ket{\psi}_{\RegW}$, the prover computes public keys $\pk_i \gets \extpk(\PK, i)$ for $1\leq i\leq N$. From now on, $P$ operates directly on $(\pk_i)$ and ignores $\PK$. 

The prover coherently (with respect to $\ket{\psi}$) computes a ``range superposition''
    \[\frac 1 {\sqrt{L^N}} \sum_{\substack{x_1, \hdots, x_N \in D \\ y_1, \hdots, y_N \in R \\ w \in \{0,1\}^N}} \left( \alpha_{w} \prod_i \sqrt{p_{\pk_i}(w_i, x_i, y_i)} \ket{w}_{\RegW} \ket{x_1}_{\RegX_1} \hdots \ket{x_N}_{\RegX_N} \ket{y_1}_{\RegY_1} \hdots \ket{y_N}_{\RegY_N}\right)
    \]
    where each $\RegX_i$ is an $\ell(\secp)$-qubit register (where $D \subset \{0,1\}^{\ell})$, and each $\RegY_i$ has basis $\{\ket{y} \}_{y \in R}$. Here, $p_{\pk}(b, x, y)$ denotes the probability density of $y$ in the distribution $f_{\pk}(b, x)$, where $p_{\pk}(b,x,y) \coloneqq 0$ for $x \in \{0,1\}^{\ell} \setminus D$. Following~\cite[Section 4.3]{FOCS:BCMVV18} the honest prover algorithm can efficiently prepare this state up to exponentially small trace distance. 
    
    
    After preparing this state, the prover measures $\RegY_1, \hdots, \RegY_N$ in the standard ($R$-)basis and sends the outcome $(y_1,\dots,y_N)$ to the verifier.

    \item The verifier sends a uniformly random challenge bit $c$. After receiving the prover response, the verifier computes each public key $\pk_i \gets \extpk(\PK, i)$ and secret key $\sk_i \gets \extsk(\SK, i)$ in order to evaluate either $\MP.\Test$ or $\MP.\Out$. 
    \item $\MP.\Open$: On challenge bit $c$, the prover operates as follows.
    \begin{itemize}
        \item If $c=0$, the prover measures $\RegW \tensor \RegX_1 \tensor \hdots \tensor \RegX_N$ in the standard basis and sends the outcome $(b_1, \hdots, b_N, x_1, \hdots, x_N)$ to the verifier. 
        \item If $c=1$, the prover instead measures $\RegW \tensor \RegX_1\tensor \hdots \tensor \RegX_N$ in the Hadamard basis, returning strings $d_1, \hdots d_N$.
    \end{itemize} 
    \item $\MP.\Test$: Given $(b_1, \hdots, b_N, x_1, \hdots, x_N)$, the verifier computes (for every $i$) $\mathsf{Check}(\pk_i, b_i, x_i, y_i)$ and rejects if any of these checks do not pass.
    \item $\MP.\Out$: Given $d_1, \hdots d_N$, the verifier outputs $N$ bits as follows. For each $i \in [N]$: 
    \begin{itemize}
        \item If $h_i = 0$, the verifier ignores $d_i$, computes $(b_i, x_i) = \Invert(\inj,\sk_i, y_i)$, and outputs $b_i$.
        \item If $h_i=1$, the verifier computes the two inverses $\{(0, x_{0,i}), (1, x_{1,i})\} \gets \Invert(\twotoone,\sk_i, y_i)$. For each $i$, the verifier checks whether $d_i\in \mathsf{Good}_{x_{0,i}, x_{1,i}}$ (corresponding to a valid equation in the $i$th slot), and if so, the verifier outputs $d_i \cdot (1, x_{0,i}\oplus x_{1,i})$. If $d_i \not\in \mathsf{Good}_{x_{0,i}, x_{1,i}}$, the verifier samples a uniformly random bit and outputs it.
    \end{itemize}  
\end{itemize}

Completeness of this protocol follows immediately from \cite{FOCS:Mahadev18a} and the pseudoindependence property of $\mathsf{BatchGen}$ (\cref{lemma:pseudoindependence}). That is, the outcome of the honest protocol execution is entirely a function of $(\pk_1, \hdots, \pk_N, \sk_1, \hdots, \sk_N)$, which by pseudoindependence is computationally indistinguishable from independent keys output by calls to $\Gen(1^\secp, \mode_i = C(i))$. In turn, as analyzed in \cite{FOCS:Mahadev18a,Vid20-course}, this output distribution is statistically close to the $h = (C(0), \hdots, C(N))$-measurement outcome on $\ket{\psi}$, In particular, there is only a negligible probability of a verifier abort.


\subsection{Analysis}

Changes to the proof: 

\begin{itemize}
    \item \cref{lemma:extractor-key-indistinguishability} now follows from the key indistinguishability property of 
    \item \cref{lemma:verifier-output} now requires a proof of (computational) indistinguishability (\cref{lemma:verifier-output-succinct} below)
    \item \cref{claim:collapsing} follows by invoking the collapsing property of $f_{\pk_j}$ given $\PK$ and $\{\sk_i, i\neq j\}$.
    \item \cref{claim:hardcore-bit} follows by invoking (1) the adaptive hardcore bit property of $f_{\pk_j}$ given $\PK$ and $\{\sk_i, i\neq j\}$, and (2) (within the proof of \cref{claim:hardcore-bit}) the computational two-to-oneness property of $f_{\pk_j}$ given $\PK$ and \emph{all} $\sk_i$. 
\end{itemize}

  \begin{claim}\label{lemma:verifier-output-succinct}
     For every basis choice $h$, we have that $D_{0,h}$ is computationally indistinguishable from $D_{\mathsf{Output}}$.
  \end{claim}
  
  \begin{proof}
    We define an alternate prover state $\ket{\psi'}$ that is computationally indistinguishable from $\ket{\psi}$, and such that the $(\{Z_j\}_{j\in S}, \{X_i\}_{i\in R})$ measurement outcomes of $\ket{\psi'}$ are \emph{identical} to $D_{\mathsf{Out}}$.
     
     The state $\ket{\psi'}$ is defined as follows: start with $\ket{\psi}$, and then for each $j\in S$, replace the register $\RegZ_j$ with (the classical string) $(b^*_j, x^*_j) = \Invert(\sk_j, y_j)$. The $(\{Z_j\}_{j\in S}, \{X_i\}_{i\in R})$ measurement outcomes now perfectly match $D_{\mathsf{Output}}$. 
     
    Thus, it suffices to show that $(\PK, \{\sk_i\}_{i\in R}, \ket{\psi'})$ is computationally indistinguishable from $(\PK, \{\sk_i\}_{i\in R}, \ket{\psi})$. First, we know that $(\PK, \{\sk_i\}_{i\in R},\ket{\psi})$ is computationally indistinguishable from the mixed state $\bsigma$ obtained from $(\PK, \{\sk_i\}_{i\in R},\ket{\psi})$ by measuring each register $\RegZ_j$ (for $j\in S$). This follows by the collapsing of each $f_{\pk_j}$ in the presence of $(\PK, (\sk_i)_{r^*_i = 1})$ (\cref{lemma:io-collapsing}).
    
    Then, $\bsigma$ is computationally indistinguishable from $\ket{\psi'}$ even given $(\PK, \sk_1, \hdots, \sk_N)$. This follows from the computational injectivity of each $f_{\pk_j}$ such that $s_j = 1$ (\cref{lemma:io-injectivity}) and the fact that $\ket{\psi}$ (and therefore $\bsigma$) passes the test round with probability $1-\negl(\secp)$; a distinguisher between $\bsigma$ and $\ket{\psi'}$ would necessarily find an inverse of some $y_j$ that is not equal to $\Invert(\sk_j, y_j)$. This completes the proof of the claim. 
    \end{proof}

==> macros.tex <==
%%%%%%%%%%%% Defining theorem-like environments %%%%%%%%%%
\ifsubmission
\else
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{property}[theorem]{Property}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\fi



\newtheorem{importedtheorem}[theorem]{Imported Theorem}
\newtheorem{informaltheorem}[theorem]{Informal Theorem}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{construction}[theorem]{Construction}
%\Crefname{importedtheorem}{Imported Theorem}{Imported Theorems}
%\Crefname{theorem}{Theorem}{Theorems}
%\Crefname{proposition}{Proposition}{Propositions}
%\Crefname{claim}{Claim}{Claims}
%\Crefname{lemma}{Lemma}{Lemmas}
%\Crefname{conjecture}{Conjecture}{Conjectures}
%\Crefname{corollary}{Corollary}{Corollaries}
%\Crefname{construction}{Construction}{Constructions}
%\Crefname{property}{Property}{Properties}

\theoremstyle{definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{notation}[theorem]{Notation}
%\Crefname{definition}{Definition}{Definitions}
%\Crefname{assumption}{Assumption}{Assumptions}
%\Crefname{notation}{Notation}{Notations}

\theoremstyle{remark}
\newtheorem{comment}[theorem]{Comment}
% \newtheorem{fact}[theorem]{Fact}

%\Crefname{question}{Question}{Questions}
%\Crefname{remark}{Remark}{Remarks}
%\Crefname{comment}{Comment}{Comments}
%\Crefname{fact}{Fact}{Facts}


%%Yael added:
\newcommand{\Gen}{\mathsf{Gen}}
\def\Eval{\mathsf{Eval}}
\newcommand{\Invert}{\mathsf{Invert}}
\def\Check{\mathsf{Check}}
\def\clawfree{\mathsf{ClawFree}}
\def\vecx{\mathbf{x}}
\def\vecy{\mathbf{y}}
\def\vecd{\mathbf{d}}
%\def\inj{\mbox{\rm \texttt{injective}}}
\def\inj{\mathsf{injective}}
\newcommand{\injective}{\inj}
%\def\twotoone{\mbox{\rm \texttt{2to1}}}
\def\twotoone{\mathsf{2}\text{-}\mathsf{to}\text{-}\mathsf{1}}

\newcommand{\Enc}{\mathsf{Enc}}
\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\ct}{\mathsf{ct}}
\newcommand{\FHE}{\mathsf{FHE}}
\newcommand{\Ext}{\mathsf{Ext}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Calligraphic and blackboard type letters.

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

% Quantum Registers
\newcommand{\RegA}{\mathcal{A}}
\newcommand{\RegB}{\mathcal{B}}
\newcommand{\RegC}{\mathcal{C}}
\newcommand{\RegD}{\mathcal{D}}
\newcommand{\RegE}{\mathcal{E}}
\newcommand{\RegF}{\mathcal{F}}
\newcommand{\RegG}{\mathcal{G}}
\newcommand{\RegH}{\mathcal{H}}
\newcommand{\RegI}{\mathcal{I}}
\newcommand{\RegJ}{\mathcal{J}}
\newcommand{\RegK}{\mathcal{K}}
\newcommand{\RegL}{\mathcal{L}}
\newcommand{\RegM}{\mathcal{M}}
\newcommand{\RegN}{\mathcal{N}}
\newcommand{\RegO}{\mathcal{O}}
\newcommand{\RegP}{\mathcal{P}}
\newcommand{\RegQ}{\mathcal{Q}}
\newcommand{\RegR}{\mathcal{R}}
\newcommand{\RegS}{\mathcal{S}}
\newcommand{\RegT}{\mathcal{T}}
\newcommand{\RegU}{\mathcal{U}}
\newcommand{\RegV}{\mathcal{V}}
\newcommand{\RegW}{\mathcal{W}}
\newcommand{\RegX}{\mathcal{X}}
\newcommand{\RegY}{\mathcal{Y}}
\newcommand{\RegZ}{\mathcal{Z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typography
\newcommand{\textdef}[1]{\textnormal{\textsf{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Complexity classes

\newcommand{\QMA}{\mathsf{QMA}}
\newcommand{\NP}{\mathsf{NP}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Cryptography notation

\newcommand{\secp}{\lambda}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\polylog}{\mathsf{polylog}}
\newcommand{\negl}{\mathsf{negl}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\mode}{\mathsf{mode}}
\newcommand{\Setup}{\mathsf{Setup}}
\newcommand{\extpk}{\mathsf{ExtPk}}
\newcommand{\extsk}{\mathsf{ExtSk}}
\newcommand{\Program}{\mathsf{Program}}
\newcommand{\PK}{\mathsf{PK}}
\newcommand{\SK}{\mathsf{SK}}
\newcommand{\iO}{\mathsf{i}\mathcal{O}}
\newcommand{\Hyb}{\mathsf{Hyb}}
\newcommand{\PRG}{\mathsf{PRG}}
%\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\bit}{\mathsf{bit}}
%\newcommand{\state}{\mathsf{st}}

% measurement protocol
\newcommand{\MP}{\mathsf{MP}} 
\newcommand{\Test}{\mathsf{Test}}
\newcommand{\Out}{\mathsf{Out}}
\newcommand{\Commit}{\mathsf{Commit}}
\newcommand{\Open}{\mathsf{Open}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Quantum
\newcommand{\SWAP}{\mathsf{SWAP}}
\newcommand{\Id}{\mathsf{Id}}

% Density matrices
\newcommand{\brho}{\bm{\rho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\tensor}{\otimes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probability

\DeclareMathOperator*{\E}{\mathbb{E}}

% !TeX root = ./0-main.tex

